Probabilistic Models for Computerized Adaptive Testing: Experiments

This paper follows previous research we have already performed in the area of Bayesian networks models for CAT. We present models using Item Response Theory (IRT - standard CAT method), Bayesian networks, and neural networks. We conducted simulated CAT tests on empirical data. Results of these tests are presented for each model separately and compared.

==> mc_conclusion.tex <==
\section{FUTURE WORK} 
In this section we present a brief overview of research problems of our further interest. 

\subsubsection*{Constrained question selection}
Adaptive tests constructed with the IRT model have various well established methods of selecting next questions. As it was discussed in the first chapter, the selection process should be carefully managed to prevent the overuse of some questions as well as very similar question combinations for many participants. One way IRT researchers are solving this issue is through a series of constraints in the selection process~\cite{VanderLinden2004,Stocking2000}. We plan to analyze the use of such constraints for BN models. The research will be conducted in order to define the correct constraints, their application and their impact on the CAT procedure.

\subsubsection*{Precision of skills measurement}
Stopping rules for CAT used in IRT are of two kinds. \begin{itemize}
	\item Practical, e.g., limited time of the test or a specific number of asked questions, or
	\item Statistical, e.g., reliability of the test (precision of measured latent skill).
\end{itemize} 
The goal of this research path is to provide a similar criteria for BN-CAT models as well. We will establish a criterion able to provide a statistically sound precision of estimates. Afterwards, we will review the effect of using this criterion as the stopping rule for CAT.

\subsubsection*{Model quality criterion}
So far in our research we were evaluating a model quality based on its predictions of answers to remaining questions. This criterion provide reasonable results but it also at the same time has some drawbacks. First of all, for some models similar to each other it is often hard to order them in terms of quality. The prediction accuracy varies over the test run and the order of models changes in different steps (different numbers of asked questions). Next, some models are able to predict the student's skills very well while their prediction power back to answers is not that good. These models have an disadvantage compared to other models (with better backwards precision) if we use the current criterion. This applies especially for some of Neural networks models. 

We will focus a part of our efforts on the design and testing criteria that are able to take into account more aspects of models for CAT. We would like to better describe and experimentally verify on data criteria that work with skills estimates. Specifically, we will measure the quality of a model as a correlation of the predicted score with the real score. Also we want to compare the final ordering of students based on predictions and real values. 

\subsubsection*{Model creation}
One reason of small spread of practical use of CAT is the high amount of work required to create a student model. The process itself may be very useful due to its highly organized character and statistically strong results, but it requires a certain level of expertise in modeling and statistics. 

We want to address an option of automated model creation based on data. Algorithms for BN structure learning in a general case exist, some examples are in~\cite{Margaritis2003}. These algorithms cover general structure learning which may serve well in some areas but in case of CAT it usually does not reflect our situation very well. We would like to explore special types of models which would fit better for our needs as the CAT model. This leads to learning a model which contains a local structure. It is an interesting theoretical task for the whole BN community, not limited only to CAT.

\subsubsection*{Local structure in BNs}
Bayesian networks encode conditional probabilities. These probabilities can be encoded in many ways. One of the most common is to define a conditional probability table (CPT). This table defines a conditional probability of a variable for every combination of its parents. For example, let us consider the network in the Figure~\ref{fig:net}. The CPT for this network with a child $Y$ and parents $X_1,X_2,X_3$ is in the Table~\ref{tab:cpt} (values are chosen at random). In the general case we have to specify $2^n$ parameters where $n$ is the number of parents. In the example case, we need $2^3 = 8$ parameters. This amount of parameters correspond to binary nodes. For nodes with more than two states, the total amount of parameters is even higher.

\begin{figure}%
\centering
\begin{tikzpicture}
  \SetGraphUnit{2.5}
	\SetUpEdge[style={->,>=biggertip}]
	\Vertex[Math,L=X_2] {X2}
 
  \EA[Math,L=X_3](X2){X3}
  \WE[Math,L=X_1](X2){X1}
	\SO[Math,L=Y](X2){Y}
  \Edge(X2)(Y)
  \Edge(X1)(Y)  
	\Edge(X3)(Y)  
	
\end{tikzpicture}
\caption{Simple Bayesian network}%
\label{fig:net}
\end{figure}


\begin{table}%
\centering
\begin{tabular}{lcccccccc}
\hline
$X_1$ & 1 & 1 & 1 & 1 & 0 & 0 &0 &0 \\
$X_2$& 1 & 1 & 0 & 0 & 1 & 1 &0 &0 \\
$X_3$& 1 & 0 & 1 & 0 & 1 & 0 &1 &0 \\
\hline
$Y(0)$ & 0.05 & 0.41 & 0.12 & 0.67 & 0.85 & 0.5 &0.9 &0.08 \\
$Y(1)$ & 0.95 & 0.59 & 0.78 & 0.33 & 0.15 & 0.5 &0.1 &0.92 \\
\hline
\end{tabular}
\caption{CPT for the BN in~\ref{fig:net}}
\label{tab:cpt}
\end{table}

If we have additional information about the structure (relations) of BN variables we can use this information to our benefit. The local structure in a BN allow us to specify these relations and encode conditional probabilities efficiently. The local structure concept is sometimes called as canonical models. A more thorough introduction to the theory of canonical models can be found in~\cite{Diez2007}. Basically, we establish a function that prescribes how to compute a child's value from its parents. The function can be of many different types, but for our illustration example, we will now consider the noisy OR function only. If there is OR local structure (without noise) it means, that the value of $Y$ is:
$$Y = X_1 \vee X_2 \vee X_3$$
Because the relation is encoded directly in the formula, there is no need to specify a CPT. In this case, we need to know only the values of $X_1,X_2,X_3$. To this model we introduce noise by adding auxiliary variables $Z_1,Z_2,Z_3$. The network then changes from the one in the Figure~\ref{fig:net} to the one in the Figure~\ref{fig:net2}. In this case we need to specify probabilities $$P(Z_i|X_i)$$which specify the noise. This forms the noisy OR local structure. The total number of parameters that we have to specify is $2n$ (there might be one additional inhibitor variable making it to $2(n+1)$ parameters). In our example case we have to specify $2\cdot 3 = 6$ or $8$ parameters. It means there is a difference of $O(n)$ for models with a local structure compared to $O(2^n)$ without a local structure.

\begin{figure}%
\centering
\begin{tikzpicture}
  \SetGraphUnit{2.5}
	\SetUpEdge[style={->,>=biggertip}]
	\Vertex[Math,L=X_2] {X2}
 
  \EA[Math,L=X_3](X2){X3}
  \WE[Math,L=X_1](X2){X1}
	\SO[Math,L=Z_1](X1){Z1}
	\SO[Math,L=Z_2](X2){Z2}
	\SO[Math,L=Z_3](X3){Z3}
	\SO[Math,L=Y,style = {double}](Z2){Y}
	\node	at ([shift=(-7cm:-1cm)]Y) (l) {OR};	
  \Edge(X2)(Z2)
  \Edge(X1)(Z1)  
	\Edge(X3)(Z3)  
	\Edge(Z2)(Y)
  \Edge(Z1)(Y)  
	\Edge(Z3)(Y)  
	
	
\end{tikzpicture}
\caption{Bayesian network with noisy OR}%
\label{fig:net2}
\end{figure}

We will explore learning strategies for BNs with a local structure. It means, we have to modify the learning process of the general BN to this special case. During the general structure learning we use criteria for the model ranking. AIC/BIC\footnote{Akaike Iformation Criterion/Bayesian Information Criterion} criteria are popular. These criteria takes into account the prediction quality of a model, but also penalize it for its size. It is necessary to adapt these criteria to the specialized case of BNs with the local structure. AIC/BIC work with the number of nodes to compute parameters, but with the local structure the reduction of number of parameters is essential. 

It is clear that exploiting a local structure in a BN has many advantages. 
\begin{itemize}
	\item First, it is easier to learn a statistically reliable model with less parameters.
	\item We are able to create more complex models where computational operation will be quickly solvable.
	\item It is possible to store this model in less space.
	\item Last but not least, we do not need to specify a large number of conditional probabilities. These probabilities are often obtained from experts and it may be difficult to get reliable estimates of them for large CPTs. With the local structure, we have to specify significantly less conditional probability values.
\end{itemize}

